Bayesian analysis and naturalness of (Next-to-)Minimal Supersymmetric Models

The Higgs boson discovery stirred interest in next-to-minimal supersymmetric models, due to the apparent fine-tuning required to accommodate it in minimal theories. To assess their naturalness, we compare fine-tuning in a $\mathbb{Z}_3$ conserving semi-constrained Next-to-Minimal Supersymmetric Standard Model (NMSSM) to the constrained MSSM (CMSSM). We contrast popular fine-tuning measures with naturalness priors, which automatically appear in statistical measures of the plausibility that a given model reproduces the weak scale. Our comparison shows that naturalness priors provide valuable insight into the hierarchy problem and rigorously ground naturalness in Bayesian statistics. For the CMSSM and semi-constrained NMSSM we demonstrate qualitative agreement between naturalness priors and popular fine tuning measures. Thus, we give a clear plausibility argument that favours relatively light superpartners.

==> PLAN.tex <==
\begin{color}{red}

\section{General outline}

\begin{enumerate}
\item Introduce idea that Bayesian statistics underpins traditional ideas about fine-tuning. 
\item Possibly include distribution of $\Lambda$, the SM cut-off, to illustrate this point.
\item Introduce idea of effective prior from integrating $Z$-boson mass measurement.
\item Present analytic formulas for effective priors in NMSSM.
\item Present two-dimensional maps of marginalized effective priors for NMSSM.
\item Compare above with Barbieri-Giudice measure.
\item Compare evidences $p(M_Z|\textrm{model})$ between models.
\end{enumerate}

\section{We need}

\begin{enumerate}
\item Make any more plots that we want (AF think we have them all) and finish results/conclusions
\item In the conclusions section, there are a lists of refs. that we *could* add to the main text or delete. 
\end{enumerate}

\end{color}
\clearpage
\setcounter{section}{0} 


==> scraps.tex <==
\begin{color}{red}

\section{Electroweak Symmetry Breaking}

The Higgs potential is given by,
\ba V_{Higgs} & = & V^H_F + V^H_D + V_{\rm soft}^H + \Delta V_{eff} \\
V_F^H&=& |\lambda S|^2 (|H_u|^2+|H_d|^2) + |\lambda H_uH_d
+\kappa S^2|^2 , \label{eq:HpotF} \\
V_D^H &=& \frac{1}{8} \bar g^2 (|H_d|^2-|H_u|^2)^2
 +\frac{1}{2}g^2|H_u^{\dagger}H_d|^2 , \label{eq:HpotD} \\
V^H_{\rm soft}&=&m_{H_u}^2|H_u|^2 + m_{H_d}^2|H_d|^2 + m_S^2|S|^2
+ [\lambda A_{\lambda}SH_uH_d+\frac{1}{3}\kappa A_{\kappa}S^3+\hc ], 
\label{eq:HpotS}
\ea where $\bar g = \sqrt{g^2+g^{\prime 2}}$ and $g$ and $g^{\prime}$
are the gauge couplings of $SU(2)_L$ and $U(1)$ interactions
respectively, with $g = g_2$ and $g^\prime = \sqrt{3/5} \, g_1$ and we have taken $H_uH_d \equiv
\epsilon_{\alpha \beta}(H_u)^{\alpha}(H_d)^{\beta}=H_u^+H_d^--H_u^0H_d^0$.  $\Delta V_{eff}$ are the higher order corrections to the Coleman-Weinberg potential, which at 1-loop gives,
\begin{equation}
	\Delta V_\textrm{eff}=\frac{1}{64\pi^2}~\textrm{STr}~\mathcal{M}^4\left[\ln\left(\frac{\mathcal{M}^2}{M_{SUSY}^2}\right)-\frac{3}{2}\right],
\end{equation}
where $\mathcal{M}=\mathcal{M}(Q=M_{SUSY})$ is the mass matrix of fields and $\textrm{STr}$ is the supertrace over all fields which gives an additional factor 1 for scalars and -2 for fermions.

The three neutral Higgs fields then pick up vacuum expectation values,  
\begin{equation} 
        \langle H_d \rangle = {v_d \choose 0}, 
\qquad  \langle H_u \rangle = {0 \choose v_u}, 
\qquad  \langle S \rangle =  s, \label{eq:potmin} \end{equation}
  
\noindent and the minimisation conditions relate the VEVs to the soft masses,

\ba m_{H_d}^2&=& \frac{1}{4} {\bar g}^2 (v_u^2-v_d^2) - \lambda^2 v_u^2
 + (A_{\lambda}  +\kappa s) \lambda s \frac{v_u}{v_d} 
- \lambda^2 s^2 - \frac{1}{2v_d}\frac{\partial \Delta  V_{eff}}{\partial v_d}, \label{eq:mind}\\
m_{H_u}^2&=& \frac{1}{4} {\bar g}^2 (v_d^2-v_u^2) -\lambda^2 v_d^2 
+ (A_{\lambda}  +\kappa s) \lambda s \frac{v_d}{v_u} 
- \lambda^2 s^2 -\frac{1}{2v_u}\frac{\partial \Delta  V_{eff}}{\partial v_u}, \label{eq:minu} \\
m_S^2 &=& -2 \kappa^2 s^2 - \lambda^2v^2 + 2 \kappa\lambda v_uv_d
+ \lambda A_{\lambda} \frac{v_uv_d}{s}
-\kappa A_{\kappa}s - \frac{1}{2s}\frac{\partial  \Delta V_{eff}}{\partial s} \label{eq:mins}
\ea
Eq.(\ref{eq:mind}, \ref{eq:minu}) can be rewritten as
\begin{eqnarray}
	\mu_\textrm{eff}^2&=&\frac{\overline{m}_{H_d}^2-\overline{m}_{H_u}^2t^2}{t^2-1}-\frac{1}{2}\overline{M}_z^2,\label{nmssm_mu}\\
	B_\textrm{eff}\mu_\textrm{eff}&=&\frac{1}{2}\sin{2\beta}\left(\overline{m}_{H_u}^2+\overline{m}_{H_d}^2+ 2\mu_\textrm{eff}^2\left(1+\frac{\overline{M}_z^2}{\overline{g}^2s^2}\right)\right)\label{nmssm_bmu}
\end{eqnarray}
with $\mu_\textrm{eff}\equiv\lambda s$ and $B_\textrm{eff}\equiv A_\lambda+\kappa s$ and we have also defined, 
\ba \overline{m}^2_{H_d} &=&  m^2_{H_d} - \frac{1}{2v_d}\frac{\partial \Delta V}{\partial v_d}, \quad
 \overline{m}^2_{H_u} =  m^2_{H_u} - \frac{1}{2v_u}\frac{\partial \Delta V}{\partial v_u}, \quad
\overline{M}_Z^2 = M_Z^2 + {\mathcal Re}\Pi_{ZZ}^T. \ea.

\subsection{Effective priors and fine tuning} 
Since the analysis is performed using a spectrum generator, NMSPEC which is part of the NMSSMTools 3.2.1 package, the parameters we vary depend on the spectrum generator.   In particular it is normal in SUSY spectrum generators to replace certain high scale\footnote{In this case high scale refers to the scale at which the parameters are set.  So in the semi-constrained version this would be the GUT scale, while in the NMSSM10 we are assuming the parameters are set at $10$ TeV, so our ``high scale'' is much lower than in the semi-constrained case.} parameters which define our models with low energy parameters some of which are known from experiment. 

  For example in the MSSM $v^2 = v_u^2 + v_d^2$ is known from experiment and we use the measured $Z$ boson mass to remove this degree of freedom.  However this means that we have one less degree of freedom as the VEV, which can been derived from the model parameters, is now essentially an input parameter, albeit one whose value is known from experiment.    The ratio of the VEVs, $\tan \beta = v_u / v_d$ is also a significant quantity as it must be specified to extract the  tree level Yukawas from the fermion masses.    

Therefore spectrum generators in the MSSM typically swap $\{\mu, m_3^2\} \rightarrow \{ M_Z^2, \tan \beta, sign(\mu) \}$, using the EWSB conditions,

 \ba \label{Mzsqpred}
\overline{M}_Z^2& =& \frac{2
(\overline{m}^2_{H_d} - \overline{m}^2_{H_u}\tan^2{\beta})}{\tan^2{\beta}-1 } - 2|\mu|^2  \rm{,} \\
\label{s2bpred} sin(2 \beta) &=&  \frac{2 B\mu}{\overline{m}_{H_u}^2 + \overline{m}_{H_d}^2 + 2 |\mu^2|}
\ea where due to $\mu$ only appearing as $|\mu|^2$ we also have the sign of $\mu$ as an additional parameter.


Initially Bayesian analyses were performed on the CMSSM, with flat and
logarithmic priors for the parameter set $\{m_0, M_{1/2}, A, \tan
\beta, sign(\mu) \}$.  However this is very different from choosing
to study the model with flat and logarithmic priors for $\{m_0,
M_{1/2}, A, \mu, m_3^2 \}$, since reparametersiation is also a way of
changing the prior distribution.

In particular one reason many physicists expect superpartner masses
to be light enough to be observed at the LHC is because very heavy
superpartner masses would imply a very large cancellation between soft
masses and the $\mu$ parameter within the electroweak symmetry
breaking conditions. In Bayesian language the problem is that there is
a very small prior volume where this cancellation takes place and
therefore the observation of $M_Z = 91.1876$ does not fit well with
our prior expectations if superpartners are heavy.  However when the
magnitude of $\mu$ is replaced by $M_Z$ as an input parameter,
choosing logarithmic or flat distributions for the remaining
parameters does not reflect this theoretical prejudice.

 Naturalness priors have been introduced to account for this.
 Initially they were defined just as an ad-hoc prior weighting
 \cite{Allanach:2007qk} but later derived as a jacobian transformation
 for the change of parameters $\{|\mu|, B\mu \} \rightarrow \{M_Z^2,
 \tan \beta\}$ \cite{Allanach:2007qk, Cabrera:2008tj,
   Ghilencea:2012gz, Ghilencea:2012qk, Fichet:2012sn}. Such priors
 have mostly been used to study the parameter space of a given the model, but
 recently they have also been used for model comparison \cite{Balazs:2012qc}.
 The jacobian transformation provides an effective prior which allows
 you to do a Bayesian treatment of the MSSM including $\mu$ and $B\mu$
 as parameters while working with a spectrum generator which trades
 these parameters for $M_Z^2$ and $\tan \beta$.

 In addition the inverse of this Jacobian transformation, which
 strongly resembles the traditional fine tuning measures used in the
 literature \cite{deCarlos:1993rbr, deCarlos:1993ca, Chankowski:1997zh,
   Agashe:1997kn, Wright:1998mk, Kane:1998im, BasteroGil:1999gu,
   Feng:1999zg, Allanach:2000ii, Dermisek:2005ar, Barbieri:2005kf,
   Allanach:2006jc, Gripaios:2006nn, Dermisek:2006py, Barbieri:2006dq,
   Kobayashi:2006fh, Perelstein:2012qg, Antusch:2012gv,Cheng:2012pe,
   CahillRowley:2012rv, Ross:2012nr, Basak:2012bd} and other fine
 tuning measures which have been proposed \cite{Anderson:1994dz,
   Anderson:1994tr, Anderson:1995cp, Anderson:1996ew,
   Ciafaloni:1996zh, Chan:1997bi, Barbieri:1998uv, Giusti:1998gz,
   Casas:2003jx, Casas:2004uu, Casas:2004gh,
   Casas:2006bd,Kitano:2005wc, Athron:2007ry, Baer:2012up}, can be
 studied on it's own as well defined measure of the fine tuning.
 Since the jacobian transformation relates the priors,\footnote{where $\mathcal{T}$ labels the transformation $\{|\mu|, B\mu \} \rightarrow \{M_Z^2, \tan
 \beta\}$. }

\begin{equation} p(m_0 , M_{1/2} , A, \mu, B\mu) =  \norm{J_{\mathcal{T}} }p(m_0 , M_{1/2} , v, \tan \beta), \end{equation}

\noindent this measure defines fine tuning as the ratio of the
priors. Specifically fine tuning is the ratio between the prior you
would use if the VEVs (in the form of $v$ and $\tan \beta$) were input
parameters, so by construction there is no unnatural cancellation to
get the VEVs at the weak scale, and the prior for the high scale
parameters (in the MSSM $p(m_0 , M_{1/2} , A, \mu, B\mu)$).  

However there is one further issue here which is worth commenting
on. The MSSM does not only suffer from the little hierarchy problem
due to a heavy Higgs of $125$ GeV, it also suffers from the
$\mu$-problem. In the MSSM there is no reason why $\mu$ should be set
to the TeV scale. If one assumes a particular mechanism to generate a
TeV scale $\mu$, this may skew the prior for $\mu$ altering fine
tuning from the little hierarchy problem as well as solving the
$\mu$-problem.  In models like the NMSSM where the the $\mu$ term is
dynamically generated due to the RG evolution, we also have new
contributions to the Higgs mass which, as discussed in the
introduction, can reduce the fine tuning.  Therefore it is very
interesting to consider a Bayesian analysis of the NMSSM where we
define the model in terms of the high scale parameters and use of a
jacobian transformation to introduce naturalness priors.

\subsubsection{A fine tuning prior}

In the NMSSM we have three VEVs, $v_u, v_d$ and $s$, and instead of
$\mu$ and $B$ as fundamental parameters we generate effective terms
$\mu_{eff} = \lambda s $ and $B_{eff} = A_\lambda + \kappa s$.  As in
the MSSM one can remove any fine tuning problems of obtaining
sufficiently light VEVs if we trade high scale parameters for the VEVs,
using our electroweak symmetry braking conditions.  Therefore one can
use the jacobian for the transformation of $\{\lambda, \kappa, m_3^2
\} \rightarrow \{M_Z,\tan\beta, s \}$ as a fine tuning measure for the
NMSSM, where $\lambda$ is fixed as part of $\mu_{eff}$ in the same $\mu$
is fixed in the MSSM, $\kappa$ is fixed as part of $B_{eff}$ similarly to $B$ in the MSSM and finally the remaining electroweak symmetry breaking condition is used to trade $s$ for $m_S$.

From Eqs.~(\ref{eq:mins}, \ref{nmssm_mu}, \ref{nmssm_bmu}), we see
\begin{equation}
	\lambda=\lambda(M_z,t_\beta,s,y),\qquad
	\kappa=\kappa(\lambda,M_z,t_\beta,s,y),\qquad
	m_S=m_S(\kappa,\lambda,M_z,t_\beta,s,y).
\end{equation} where $t_\beta = \tan \beta$. The Jacobian can we then want is,
\begin{eqnarray}
	\norm{J_{\mathcal{T}_{\lambda\kappa m_S}}}&=&
	\begin{Vmatrix}
		\fp{\lambda}{M_z^2}&\fp{\kappa}{M_z^2}&\fp{m_S^2}{M_z^2}\\
		\fp{\lambda}{t_\beta}&\fp{\kappa}{t_\beta}&\fp{m_S^2}{t_\beta}\\
		\fp{\lambda}{s}&\fp{\kappa}{s}&\fp{m_S^2}{s}
	\end{Vmatrix}_{m_0,m_{1/2},A_\lambda,A_\kappa}\label{J_nmssm}
\end{eqnarray}

 
The elements in this Jacobian can be found by differentiating Eq.~(\ref{nmssm_mu},\ref{nmssm_bmu},\ref{eq:mins}).   Doing the differentiation and rearranging slightly yields
\begin{eqnarray}
	d\lambda&=&\fp{\lambda}{s}ds+\fp{\lambda}{t_\beta}dt_\beta+\fp{\lambda}{M_z^2}dM_z^2
        \\ \label{dlambda} &=& b_1ds+b_2dt_\beta+b_3dM_z^2, \end{eqnarray}
and similarly \begin{eqnarray}\label{dkappa} 0 &=& e_0d\lambda+ e_1ds
  + e_2dt_\beta + e_3dM_z^2 +e_4d\kappa, \\
\label{dms1}	dm_S^2
	&=&a^s_0d\lambda + a^s_1ds + a^s_2dt_\beta + a^s_3dM_z^2 +
a^s_4d\kappa.
\end{eqnarray} where the coefficients are given in the Appendix.

% subsection jacobian_of_t__lambdakappa_m_S_ (end)
It is also useful to express Eq.~(\ref{dms1}) by substituting in for $d \lambda$ and $d\kappa$ since we are interested initially in the case where they are functions of the parameters $s$, $t$ and $M_Z^2$. We then get $dm_S$ in terms of new coefficients,
\begin{eqnarray}
	dm_S^2&=& f_1ds + f_2dt_\beta + f_3dM_z^2.\label{dms2}
\end{eqnarray}

{\color{red}\it{ Have removed y dependence since we set that to zero anyway.}}

The jacobian can then be obtained by inserting the appropriate derivatives, giving 
\begin{eqnarray}
	J_{\mathcal{T}_{\lambda\kappa m_S}}&=&
	\begin{vmatrix}
		\fp{\lambda}{M_z^2}&\fp{\kappa}{M_z^2}&\fp{m_S^2}{M_z^2}\\
		\fp{\lambda}{t_\beta}&\fp{\kappa}{t_\beta}&\fp{m_S^2}{t_\beta}\\
		\fp{\lambda}{s}&\fp{\kappa}{s}&\fp{m_S^2}{s}
	\end{vmatrix}\\
	&=&
	\begin{vmatrix}
		\fp{\lambda}{M_z^2}&-\frac{1}{e_4}\left(e_0\fp{\lambda}{M_z^2}+e_3\right)&f_3\\
		\fp{\lambda}{t_\beta}&-\frac{1}{e_4}\left(e_0\fp{\lambda}{t}+e_2\right)&f_2\\
		\fp{\lambda}{s}&-\frac{1}{e_4}\left(e_0\fp{\lambda}{s}+e_1\right)&f_1
	\end{vmatrix}\end{eqnarray} and by use of Gaussian elimination this can be simplified to
\begin{eqnarray}	% &=&-\frac{b_3f_1-b_1f_3}{b_3}\frac{(a^s_2b_3-a^s_3b_2)(e_1b_3-e_3b_1)-(e_2b_3-e_3b_2)(a^s_1b_3-a^s_3b_1)}{a^s_4(e_1b_3-e_3b_1)-e_4(a^s_1b_3-a^s_3b_1)}\\
	% &=&\frac{(a^s_2b_3-a^s_3b_2)(e_1b_3-e_3b_1)-(e_2b_3-e_3b_2)(a^s_1b_3-a^s_3b_1)}{b_3 e_4}\\
	&=&\begin{vmatrix}
		&b_1&e_1&a^s_1&\\
		&b_2&e_2&a^s_2&\\
		&b_3&e_3&a^s_3&
	\end{vmatrix}.
\end{eqnarray} or with some manipulation of the partial derivatives, exploiting Eq.~(\ref{eq:mind}-\ref{eq:mins}), we can reorganize the dependence of each parameter to
\begin{equation}
	\lambda=\lambda(M_z,t_\beta,m_S),\qquad
	\kappa=\kappa(\lambda,t_\beta,m_S),\qquad
	m_S=m_S(M_z,t_\beta,s),
\end{equation} which allows the result to be expressed in particularly elegant form,
\begin{eqnarray}	\norm{J_{\mathcal{T}_{\lambda\kappa m_S}}}&=&\left.\fp{\lambda}{M_z^2}\right|_{t_\beta,m_S} \left.\fp{\kappa}{t_\beta}\right|_{\lambda,m_S} \left.\fp{m_S^2}{s}\right|_{M_z,t_\beta}.\end{eqnarray}

To take the MSSM limit of the NMSSM we want to decouple $S$ from $H_u$ and $H_d$, while ensuring $\mu_{eff} = \lambda s$ and $B_{eff} = A_\lambda+\kappa s$,
 remain finite.  To do this we take $\lambda, \lambda\kappa, \lambda A_\lambda\to0$ to decouple the singlet and then we must take $s  \rightarrow  \infty$ such that $\mu, B\mu$ remain finite. 
        
 Now note that multiplying $B$ by $\lambda$ along with then taking both $\lambda A_\lambda \rightarrow 0$ and $\lambda \rightarrow 0$ implies that $\kappa \rightarrow 0$ as well.  So the MSSM limit is given by

\begin{eqnarray}
  	\lambda, \kappa, \lambda A_\lambda&\to&0 \\
        s & \rightarrow & \infty.
\end{eqnarray} such that \begin{eqnarray}
	\lambda s &=& \mu,\\
	A_\lambda+\kappa s &=& B,
\end{eqnarray} remain finite. The single MSSM soft bilinear mass $B$ is obtained from the NMSSM by both $A_\lambda$ and $\kappa s$, which remains finite, and so has a redundant degree of freedom.  The singlet mass $m_S$ and trilinear $A_\kappa$ are not involved here and due to the decoupling they affect only the decoupled singlet sector, playing no role in the physics of the MSSM. However to ensure the decoupled singlet potential has a global minimum with a non-zero VEV for $S$, one should also impose that $A_\kappa > 9 m_S^2$\cite{Ellwanger:1996gw}. 



We can see that in this MSSM limit this Jacobian becomes block
diagonal.  The upper left two by two block part,
$J_{\mathcal{T}_{\lambda\kappa}}$ can then easily be related to that
of the MSSM, $J_{\mathcal{T}}$,

\begin{eqnarray}
	J_{\mathcal{T}} &=&
	\begin{vmatrix}
		\fp{\mu}{M_z^2}&\fp{B}{M_z^2}\\
		\fp{\mu}{t_\beta}&\fp{B}{t_\beta}
	\end{vmatrix}
	=s^2\begin{vmatrix}
		\fp{\lambda}{M_z^2}&\fp{\kappa}{M_z^2}\\
		\fp{\lambda}{t_\beta}&\fp{\kappa}{t_\beta}
	\end{vmatrix}_{s,A_\lambda}
	=s^2J_{\mathcal{T}_{\lambda\kappa}^s}.
\end{eqnarray}

When first we consider only the two parameter case with the logarithmic prior and take the MSSM limit,
\begin{equation}
	\frac{d\lambda
          d\kappa}{\lambda\kappa}\xrightarrow{\textrm{keep
            $s$}}J_{\mathcal{T}_{\lambda\kappa}}\frac{dM_z^2dt_\beta}{\lambda\kappa}\xrightarrow{\textrm{MSSM}}
        J_{\mathcal{T}}\frac{dM_z^2dt_\beta}{\lambda\kappa
          s^2}\overset{\textrm{shift}}{\xrightarrow{A_\lambda \to 0}}\frac{d\mu dB}{\mu B}
\end{equation}
where we have obtained the MSSM Jacobian in the last step by removing the redundant parameter $A_\lambda \rightarrow 0$.  This extra requirement should not be surprising since $\kappa$ is explicitly playing the role that $B$ does in our NMSSM Jacobian.  So far we only considered the Jacobian for the transformation of the first two EWSB conditions, thus mirroring the MSSM case. However in the NMSSM the  the third EWSB condition could be used to exchange $m_S$ for the singlet VEV $s$.  Then we get,
\begin{eqnarray}
	\frac{d\lambda d\kappa dm_S^2}{\lambda\kappa m_S^2}&=&
        J_{\mathcal{T}_{\lambda\kappa}}\frac{dM_z^2dt_\beta dm_S^2}{\lambda\kappa
          m_S^2}\xrightarrow{MSSM}
        \left[-\frac{1-t_\beta^2}{4t(1+t_\beta^2)}\frac{B}{s^2\kappa\mu^2}\right]dM_z^2dt_\beta ds
        +\mathcal{O}(A_\kappa^{-1})\label{mssm_limit_of_full_jacobian}\\ &=&
        \xrightarrow[A_\kappa \to \infty]{A_\lambda \to 0}
        \frac{d\mu dB ds}{\mu Bs}.
\end{eqnarray} Here although we take the MSSM limit, we are still including a change of variables in the decoupled singlet sector, so it is not surprising that in the last step we must also take $A_\kappa$ to infinity to obtain the MSSM Jacobian.  


Thus in the NMSSM parameter space, if we play on a slice of the MSSM
hyper surface, the Jacobian converges to the MSSM case with the
appropriate limit taken.  That is,
\begin{eqnarray}
	&&\int_\textrm{NMSSM}
  \mathcal{L}~\textrm{Pr}(m_0,m_{1/2},A_0;A_\lambda,A_\kappa)dm_0
  dm_{1/2} dA_0 \left(dA_\lambda dA_\kappa\right)\frac{d\lambda
    d\kappa dm_S^2}{\lambda\kappa
    m_S^2}\notag\\ &=&\int_\textrm{NMSSM}
  \mathcal{L}~\textrm{Pr}(m_0,m_{1/2},A_0)dm_0 dm_{1/2}
  dA_0\left[\int_\textrm{NMSSM/MSSM}+\int_\textrm{MSSM}\right]
  \frac{d\lambda d\kappa dm_S^2}{\lambda\kappa
    m_S^2}\notag\\ &=&\int_\textrm{NMSSM/MSSM}
  \mathcal{L}~\textrm{Pr}(p_\textrm{NMSSM})dp_\textrm{NMSSM}\notag\\ &&+
  \int_\textrm{MSSM} \mathcal{L}~\textrm{Pr}(m_0,m_{1/2},A_0)dm_0
  dm_{1/2} dA_0 \frac{d\mu dB ds}{\mu B
    s}\\ &=&\int_\textrm{NMSSM/MSSM}
  \mathcal{L}~\textrm{Pr}(p_\textrm{NMSSM})dp_\textrm{NMSSM} + S
  \int_\textrm{MSSM}
  \mathcal{L}~\textrm{Pr}(p_\textrm{MSSM})dp_\textrm{MSSM}.
\end{eqnarray}
Here $S$ factor in the last line stands for the integration (marginalization) factor which is a constant if the likelihood is independent of $s$. Or, some specific number taken by the MSSM limit of irrelevant parameters such as $s$ or $m_S^2$.

\subsubsection{Comparison with the traditional Fine-tuning measure} % (fold)
\label{sub:fine_tuning_measure_with_respect_to_m_z_2_}

This can also be compared to the traditional fine tuning measure.
\begin{equation}
	c_{p_i}=  \frac{p_i}{M_z^2} \fp{M_z^2}{p_i} =\fp{\log{M_z^2}}{\log{p_i}}.
\end{equation}


% = \left(\left.\fp{M_z^2}{\lambda}\right|_{\kappa,m_S^2},
%   \left.\fp{M_z^2}{\kappa}\right|_{\lambda,m_S^2},
%   \left.\fp{M_z^2}{m_S^2}\right|_{\lambda\kappa}\right)

Expressing $dm_S^2$ as,
{\allowdisplaybreaks
\begin{eqnarray}
	dm_S^2
	&\equiv& h_0 d\lambda+ h_3 dM_z^2+h_4 d\kappa,
\end{eqnarray}} where the coefficients are given in the appendix, allows us to immediately right down,
\ba
c_\lambda &=& \left.\fp{\log{M_z^2}}{\log{\lambda}}\right|_{\kappa, m_S^2} = -\frac{h_0\lambda} {h_3 M_z^2}, \\
&\xrightarrow{\textrm{MSSM}}&
 -4\frac{\mu^2}{M_z^2}\left[1-\frac{t_\beta^2(1+t_\beta^2)}{(t_\beta^2-1)^3}\frac{m_{H_d}^2-m_{H_u}^2}{B\mu}\left(\frac{B}{\mu}-\frac{4t_\beta}{1+t_\beta^2}\right)\right]=c_\mu^\textrm{MSSM},	
	\ea  thus matching the MSSM in the appropriate limit.

{\color{red}\it{to be finished...}}


\subsubsection{Effective priors for use with NMSSMTools} % (fold)
\label{sec:fine_tuning_study_with_nmssmtools}

Independent of the theoretical and conceptual issues, the
numerical analysis cannot be done without the spectrum generators such
as NMSSMTools. For the semi-constrained version of the NMSSM NMSSMTools
treats $M_z$ and $\tan\beta$ as the input parameters, using the EWSB
conditions to trade $\kappa$ and $m_S^2$ for them.  Note however this
exploits all three EWSB conditions since Eq.~\ref{Mzsqpred} is used to
trade $M_Z$ for $s$, while in Eq.~\ref{s2bpred} $\tan \beta$ is traded
for $\kappa$ and finally $m_S^2$ is fixed in the final equation, since
$s$ is already fixed by Eq.~\ref{Mzsqpred}.

The effective input parameters we can control are therefore,
$(\lambda, M_z^2, t_\beta)$, so we need the Jacobian expression
for the transformation
\begin{equation}
	J_{\mathcal{T}_{\kappa m_S}}=
	\begin{vmatrix}
		\fp{\kappa}{M_z^2}&\fp{m_S^2}{M_z^2}\\
		\fp{\kappa}{t_\beta}&\fp{m_S^2}{t_\beta}
	\end{vmatrix}_\lambda,
\end{equation}
such that we can quantify
\begin{equation}
	d\lambda d\kappa dm_S^2 = J_{\mathcal{T}_{\kappa m_S}}d\lambda dM_z^2 dt_\beta,
\end{equation}
or
\begin{equation}
	d\log\lambda~d\log\kappa~d\log m_S^2 = \frac{M_z^2 t_\beta}{\kappa m_S^2} J_{\mathcal{T}_{\kappa m_S}}d\log\lambda~d\log M_z^2~d\log t_\beta.
\end{equation}

Note the $J_{\mathcal{T}_{\kappa m_S}}$ corresponds to the upper-right $2\times2$ matrix of $J_{\mathcal{T}_{\lambda\kappa m_S}}$, except that $\lambda$ should be kept constant and $s$ is variant. Using the Gaussian elimination, we can reduce the expression simple:
\begin{eqnarray}
	J_{\mathcal{T}_{\kappa m_S}}&=&
	\begin{vmatrix}
		\fp{\kappa}{M_z^2}&\fp{m_S^2}{M_z^2}\\
		\fp{\kappa}{t_\beta}&\fp{m_S^2}{t_\beta}
	\end{vmatrix}_\lambda
	=
	\begin{vmatrix}
		\fp{\kappa}{M_z^2}&h_3\\
	\fp{\kappa}{t_\beta}& 0 
	\end{vmatrix}_\lambda.
\end{eqnarray}
Thus, keeping Yukawa maintained, 
\begin{eqnarray}
	J_{\mathcal{T}_{\kappa m_S}}&=-&h_3\left.\fp{\kappa}{t_\beta}\right|_{\lambda,M_z}= \frac{h_3}{b_1e_4} (b_1e_2-b_2e_1)\\
	&=&\frac{1}{b_1}
	\begin{vmatrix}
		&b_1&e_1&a^s_1&\\
		&b_2&e_2&a^s_2&\\
		&b_3&e_3&a^s_3&
	\end{vmatrix} = \frac{1}{b_1} J_{\mathcal{T}_{\lambda\kappa m_S}}.
\end{eqnarray}
\noindent The remarkable similarity to $J_{\mathcal{T}_{\lambda\kappa m_S}}$ can be understood by considering two successive jacobian transformations which are equivalent to $\mathcal{T}_{\lambda\kappa m_S}$,
\begin{equation}
	\lambda~\kappa~m_S^2 \underset{J_{\mathcal{T}_{\kappa m_S}}}{\xrightarrow{\mathcal{T}_{\kappa m_S}}}\lambda ~M_z^2~t_\beta \underset{b_1}{\xrightarrow{\mathcal{T}_{\lambda}^{M_z t}}} M_z^2~t_\beta~s.
\end{equation}

The relative factor $b_1 = -\lambda / s = -\mu / s^2$ appears as a
result of the transformation $\lambda\to s$. Since we have shown that for logarithmic priors $\mathcal{T}_{\lambda\kappa m_S}$ in the MSSM limit gives an effective prior that matches the one needed for MSSM studies,  this factor relates the jacobian we need to use with NMSSMTools here, to the jacobian factor one would use in the MSSM.

So to perform a Bayesian scan of the semi-constrained NMSSM with NMSSMTools, model parameters $\kappa$ and $m_S^2$ are replaced with $M_z$, $\tan\beta$.  This introducing an effective prior derived from Jacobian transformation, such that,
\begin{eqnarray}
	\int_\textrm{NMSSM}\mathcal{L}p(\lambda,\kappa,m_S^2)~d\lambda d\kappa dm_S^2 &\longrightarrow& \int_\textrm{NMSSM}\mathcal{L}p(\lambda,\kappa,m_S^2)~J_{\mathcal{T}_{\kappa m_S}}~d\lambda dM_z^2 dt_\beta,\\
	\lambda~\kappa~m_S^2&\xrightarrow{J_{\mathcal{T}_{\kappa m_S}}}& \lambda~M_z~t~(\textrm{Input}\to\textrm{Spectrum Generator}\to\textrm{Multinest})\notag
\end{eqnarray}
where $p(\lambda,\kappa,m_S^2)$ is the prior probability for the corresponding parameters.


In principle this transformation could also be usable in an analysis
of the NMSSM10, since one could impose the EWSB conditions in the same
way.  However the default choice in NMSPEC/NMSSMTOOLS for models where
all the parameters are input at low energies without high scale
constraints on the soft Higgs masses is to use the EWSB conditions in
the most direct way, exchanging the VEVs for the three soft Higgs
masses, \begin{equation} \mathcal{T}_{m_{H_u} m_{H_d} m_S}:\;\; \{m_{H_u}, m_{H_d},
m_S \} \rightarrow \{m_{Z}, \tan \beta, s \}. \end{equation}

Therefore we also need the Jacobian for this transformation,  

\begin{eqnarray}
	J_{\mathcal{T}_{\kappa m_S}}
	&=&
	\begin{vmatrix}
		& a_1^{u} & a_{2}^{u}  & a_{3}^{u}   &\\
		& a_1^{d} &  a_{2}^{d} & a_{3}^{d}  &\\
		& a_1^s  &  a_{2}^s  & a_{3}^s  &
	\end{vmatrix},
\end{eqnarray} where the coefficients are given in the Appendix.




\section{High scale constraints}
The second question which we discussed a lot was what model constraints are we working with.  the usual defintion people keep in mind when the talk about a constrained model is one where all soft scalar masses at $M_X$ are $m_0$, all soft gaugino masses are $M_{1/2}$ and all trilinear soft couplings are $A$. Since, unlike the MSSM we do not have a $\mu$ and $B_\mu$ we have the following fundamental parameters 

\begin{equation}{\rm cNMSSM \, fundamental} \;\;\; \{m_0, M_{1/2}, A, \lambda, \kappa, g_0, \mathbf{y_u}, \mathbf{y_d}, \mathbf{y_e} \} \end{equation}

The $g_0$ parameter will be fixed by the gauge couplings and the RG evolution, while the yukawas will be fixed from the quark and lepton masses, the ratio of Higgs vevs and RG evolution, and as aresult ewill drop out of the list of free parameters.

Between $M_X$ and $M_Z$ we use run the parameters according to the RGEs to obtain low enregy values for all soft breaking masses at $M_Z$, and $\lambda(M_Z)$ and $\kappa(M_Z)$.




\section{EWSB}
At values of some these parameters feed into the Higgs potential,

\begin{equation} V_H = V_H^{T} + \Delta_V \;\;  V^{T}_H = V_F+V_D+V_{\rm soft} = V^{T}_H(s, v_u, v_d, \lambda, \kappa, A_\lambda, A_\kappa, m_{H_u}, m_{H_d}, m_S, g_1, g_2)\label{eq:Hpot} \end{equation}
with
\begin{equation} 
        \langle H_d \rangle = \frac{1}{\sqrt{2}} {v_d \choose 0}, 
\qquad  \langle H_u \rangle = \frac{1}{\sqrt{2}} {0 \choose v_u}, 
\qquad  \langle S \rangle = \frac{1}{\sqrt{2}} s, \label{eq:potmin} \end{equation}
  

\ba
V_F&=& |\lambda S|^2 (|H_u|^2+|H_d|^2) + |\lambda H_uH_d
+\kappa S^2|^2 , \label{eq:HpotF} \\
V_D &=& \frac{1}{8} \bar g^2 (|H_d|^2-|H_u|^2)^2
 +\frac{1}{2}g^2|H_u^{\dagger}H_d|^2 , \label{eq:HpotD} \\
V_{\rm soft}&=&m_{H_u}^2|H_u|^2 + m_{H_d}^2|H_d|^2 + m_S^2|S|^2
+ [\lambda A_{\lambda}SH_uH_d+\frac{1}{3}\kappa A_{\kappa}S^3+\hc ], 
\label{eq:HpotS}
\ea
where $\bar g = \sqrt{g^2+g^{\prime 2}}$ and $g$ and $g^{\prime}$
are the gauge couplings of $SU(2)_L$ and $U(1)$ interactions
respectively, with $g = g_2$ and $g^\prime = \sqrt{3/5} \, g_1$ and we have taken $H_uH_d \equiv
\epsilon_{\alpha \beta}(H_u)^{\alpha}(H_d)^{\beta}=H_u^+H_d^--H_u^0H_d^0$.  

The EWSB minimisation equations the provide three constraints,

\ba m_{H_d}^2&=& \frac{1}{8} {\bar g}^2 (v_u^2-v_d^2) -\frac{1}{2} \lambda^2 v_u^2
 + \frac{1}{2}(\sqrt{2} A_{\lambda}  +\kappa s) \lambda s \frac{v_u}{v_d} 
- \frac{1}{2} \lambda^2 s^2 - \frac{\partial \Delta_V}{\partial v_d}, \label{eq:mind}\\
m_{H_u}^2&=& \frac{1}{8} {\bar g}^2 (v_d^2-v_u^2) -\frac{1}{2} \lambda^2 v_d^2 
+ \frac{1}{2}(\sqrt{2} A_{\lambda}  +\kappa s) \lambda s \frac{v_d}{v_u} 
- \frac{1}{2} \lambda^2 s^2 - \frac{\partial \Delta_V}{\partial v_u}, \label{eq:minu} \\
m_S^2 &=& -\kappa^2 s^2 -\frac{1}{2}\lambda^2v^2 +\kappa\lambda v_uv_d
+\frac{1}{\sqrt{2}} \lambda A_{\lambda} \frac{v_uv_d}{s}
-\frac{1}{\sqrt{2}} \kappa A_{\kappa}s - \frac{\partial \Delta_V}{\partial s} \label{eq:mins}
\ea
  
Since the softmasses and Yukawas at low energies are functions of the fundametal GUT scale parameters we can rewrite this as,  
   \ba 
V^{T}_H & = &  V^{T}_H(s, v_u, v_d, \lambda, \kappa, A_\lambda, A_\kappa, m_{H_u}, m_{H_d}, m_S) \\ 
 & = &   V^{T}_H(s, \tan \beta, M_Z, \lambda, \kappa, A, m_0, M_{1/2}). 
\label{eq:Hpot-fund} 
 \ea 
 where for clarity we have dropped the gauge couplings which are fixed from experiment ands rewritten $v_u$ and $v_d$ as the ratio $\tan \beta \equiv v_u/v_d$ and  the magnitude $v = \sqrt{v_d^2 + v_u^2}$ and then replace $v$ with $M_Z$ to emphasis that this is fixed by experiment.


The EWSB conditions must fix three of the parameters appearing in the Higgs potential.   If we wish to use the universal soft masses as input parameters as is done for the cMSSM then one must have three from $\{\lambda, \kappa, \tan \beta, s \}$ as to be fixed by EWSB rather appearing as input parameters. Thus one mus =t either have $\lambda$ or $\tan \beta$ as an output in the iteration.  But tehse should strongly affect the RG evolution at the outset and could lead to non-convergence of the iteration in a significant region of the parameter space.

Instead NMSPEC enlarges the set of funfdamental parameters, creating what I will call the semi-constrained NMSSM (scNMSSM), to include a soft singlet mass $m_S(M_X)$ indpendent of $m_0$ and additional (though actually not necessary for this purpose) a trilinear $A_\kappa(M_X)$ soft mass independent of $A$,


\begin{equation}{\rm scNMSSM \, fundamental} \;\;\; \{m_0, m_S, M_{1/2}, A, A_\kappa, \lambda, \kappa, g_0, \mathbf{y_u}, \mathbf{y_d}, \mathbf{y_e} \} \end{equation}
    
Then we have,

     \ba 
V^{T}_H & = &  V^{T}_H(s, v_u, v_d, \lambda, \kappa, A_\lambda, A_\kappa, m_{H_u}, m_{H_d}, m_S) \\ 
 & = &   V^{T}_H(s, \tan \beta, M_Z, \lambda, \kappa, A, A_\kappa, m_0, M_{1/2}, m_S). 
\label{eq:scNMSSM-Hpot-fund} 
 \ea 

and NMSPEC then outputs $\kappa$, $s$ and $m_S$ from the EWSB conditions.


This leaves the following as minimal input parameters

\begin{equation} {\rm NMSPEC \, vscNMSSM \, inputs} \;\;\; \{m_0, M_{1/2}, A, \lambda, sign(\mu_{eff}) \} \end{equation}
 with the option to chosses $A_\kappa$ seperately from $A$ if one wishes an addistional parameter

\begin{equation} {\rm NMSPEC \, scNMSSM \, inputs} \;\;\; \{m_0, M_{1/2}, A, A_\kappa, \lambda, sign(\mu_{eff}) \} \end{equation}


\section{Fine Tuning}
From the tree level EWSB conditions one can take the combination $m_{H_d}^2 - (\tan \beta)^2 m_{H_u}^2$, noting that $M_Z^2 = \frac{1}{4} \bar{g}^2 v^2$ and also observing that the new NMSSM terms (the second term and second part of the third term) vanish one obtains an expression for $M_Z^2$ which is almost the same as the MSSM, but with $\mu \rightarrow \mu_{eff}$.

\ba M_Z^2 \approx \frac{2(m_{H_d}^2 - \tan^2\beta m_{H_u}^2)}{\tan^2\beta -1} -2 \mu_{eff} \ea


One way to include a fine tuning prior is to define a fine tuning measure, the traditional one would be,

\begin{equation} \triangle^{p_i}_{BG} = \frac{p_i}{M_Z}\frac{\partial M_Z}{\partial p_i} \end{equation}

and choosing $\triangle_{BG} = max(\{ \triangle^i_{BG}\})$.  The =n take this tuning measure and use $\frac{1}{\triangle^{p_i}_{BG}}$ as the prior for $p_i$ as was done in http://arxiv.org/abs/hep-ph/0601089.

   
However in our meeting I think we all kept in mind the more sophisticated approach of http://arxiv.org/abs/0705.0487 where they take what we view as fundamental parameters of the model with a flat distribution and then pick up a non-flat prior when we switch to the set including $M_Z$ (so that it's measured value can be input), since changing the parameterisation is equivalent to changing the prior distribution.   

For this we do not want just the fine tuning equation we want a mapping between the fundamental parameters and the input parameters (including experimenatlly fixed $M_Z$).  In the MSSM this is a map from $\{m_0, M_{1/2}, A, sign(\mu), |\mu|, B_\mu \}$ to $\{m_0, M_{1/2}, A, \tan \beta, M_Z, sign(\mu) \}$.

To do so we use a rewriting of the EWSB conditions as,

\ba \mu  & \approx & \frac{m_{H_d}^2 - \tan^2\beta m_{H_u}^2}{\tan^2\beta -1} -\frac{1}{2} M_Z^2  \\
B\mu & \approx & \frac{1}{2} \sin{2\beta} (m_{H_d}^2 + m_{H_u}^2 + 2 \mu^2)
\ea


For the NMSSM with NMSPEC it seems we would want to go from $\{  A, A_\kappa, m_0, M_{1/2}, m_S, \lambda, \kappa\}$ to $\{m_0, M_{1/2}, A, A_\kappa, \lambda,  M_Z, \tan\beta \}$.  Note that in this case the singlet vev, which is not a ``fundamental'' parameter from the model point of view is also derived quantity.

The NMSSM EWSB equations are often rewritten as,
\ba \mu_{eff}  & \approx & \frac{m_{H_d}^2 - \tan^2\beta m_{H_u}^2}{\tan^2\beta -1} -\frac{1}{2} M_Z^2  \\
B\mu_{eff} & \approx & \frac{1}{2} \sin{2\beta} (m_{H_d}^2 + m_{H_u}^2 + 2 \mu^2) \\
m_S^2 &=& -\kappa^2 s^2 -\frac{1}{2}\lambda^2v^2 +\kappa\lambda v_uv_d
+\frac{1}{\sqrt{2}} \lambda A_{\lambda} \frac{v_uv_d}{s}
-\frac{1}{\sqrt{2}} \kappa A_{\kappa}s
\ea
where $B\mu_{eff} = \sqrt{2} A_\lambda + \kappa s$ and the last equation is unchanged.   The firts of these can be seen as suitable for fixing $\mu_{eff} = \frac{1}{2}\lambda s $ or equvalently $s$ since $\lambda$ is given by the input parameters, while the second fixes $B\mu_{eff}$ or eqivalently $\kappa$.   However we are the left with an equation for $m_S^2$ which is a quadratic function of $\kappa$. 


\section{Results}
\section{Conclusions}

\clearpage
\begin{appendix}
\section{Effective prior coefficients}
\setcounter{equation}{0} \def\theequation{A.\arabic{equation}} Here we
present the coefficients that appear in the fine tuning priors.  The
coefficients appear when we differentiate the EWSB conditions, given in
Eqs.~(\ref{eq:mind}-\ref{nmssm_bmu}).  First for convenience we
reproduce the derivatives written in terms of the coefficients, in
this case in initially allowing all of the set $\{m_{H_d}, m_{H_u},
m_S, \lambda, \kappa, s, t_\beta \equiv \tan\beta, M_Z^2\}$ to vary.

\ba dm_{H_u}^2 &=&  a^u_0d\lambda + a_1^{u}\, ds + a_{2}^{u}\,dt_\beta + a_3^{u}\,dM_Z^2 + a^u_4 d\kappa \\
 dm_{H_d}^2 &=&  a^d_0d\lambda +  a_1^{d} \, ds + a_2^{d}\, dt_\beta + a_3^{d}\, dM_Z^2 +  a^d_4 d\kappa \\
 \label{Ap:dms1} dm_S^2&=&a^s_0d\lambda + a^s_1ds + a^s_2dt_\beta + a^s_3dM_z^2  +  a^s_4 d\kappa \\
  d\lambda &\equiv& b_1ds+b_2dt_\beta+b_3dM_z^2, \\
0 &\equiv& e_0d\lambda+ e_1ds + e_2dt_\beta + e_3dM_z^2 +e_4d\kappa,
\ea  where the last two lines come from the linear combinations of the EWSB conditions, written to relate $\mu_{eff}$ and $B_{eff}$, so the $b_i$ and $e_i$ should be linear combinations of the $\{a_i^d\}$ and $\{a_i^u\}$. 

Writing the trigonometric functions as $t_\beta \equiv \tan \beta, s_\beta \equiv \sin \beta, c_\beta \equiv \cos\beta$ and defining $m_3^2 \equiv B_{eff}\mu_{eff}$ the coefficients are,

\ba a_1^{u} & = & - \fp{\mu_{eff}^2}{s} + \frac{1}{t_\beta} \fp{m_3^2}{s} \hspace{4mm} 
a_{3}^{u}  = - \lambda^2 c_\beta^2 \frac{v^2}{M_Z^2} + \frac{c_{2\beta}}{2}  \hspace{4mm} 
a_{2}^{u}  = - \lambda^2 v^2 \fp{c_\beta^2}{t_\beta} + \frac{M_Z^2}{2} \fp{c_{2\beta}}{t_\beta} - \frac{m_3^2}{t_\beta^2}  \hspace{1cm} \\ 
a_1^{d} & = & - \fp{\mu_{eff}^2}{s} + t_\beta \fp{m_3^2}{s} \hspace{4mm} 
a_{2}^{d} = - \lambda^2 v^2 \fp{s_\beta^2}{t_\beta} - \frac{M_Z^2}{2} \fp{c_{2\beta}}{t_\beta} + m_3^2 \hspace{4mm} 
a_{3}^{d} =  - \lambda^2 s_\beta^2 \frac{v^2}{M_Z^2} - \frac{c_{2\beta}}{2} 
 \\
a_1^s &=& - \kappa A_\kappa - 4 \kappa^2 s - \frac{\lambda A_\lambda v^2 s_{2\beta}}{2 s^2} \hspace{4mm}  a^s_{2} =  \lambda \kappa v^2 \fp{ s_{2\beta}}{t_\beta} + \frac{\lambda A_\lambda v^2 }{2 s } \fp{ s_{2\beta}}{t_\beta} \hspace{4mm} \\
a^s_{3}& =& - \frac{\lambda^2 v^2}{M_Z^2} + \lambda \kappa s_{2\beta}\frac{ v^2}{M_Z^2} + \frac{\lambda A_\lambda v^2 s_{2\beta}}{2 s M_Z^2}
 \ea



\ba a_0^u &=& -\lambda^2 s^2 (v^2 c_\beta^2 + s^2) + \frac{A_\lambda + \kappa s}{t_\beta} s  \hspace{1cm}     a_4^u = \lambda s^2 t_\beta \hspace{1cm} \\
 a_0^d &=& -\lambda^2 s^2 (v^2 s_\beta^2 + s^2) + (A_\lambda + \kappa s) s t_\beta \hspace{1cm}     a_4^d = \frac{\lambda s^2}{t_\beta}\hspace{1cm}  \\
 a_0^s &=&  -\frac{4M_z^2}{\bar{g}^2s}\left[\lambda s-\frac{t_\beta}{1+t_\beta^2}(A_\lambda+\kappa s)\right]   \hspace{1cm}  a_4^s = -\left[4\kappa s^2+sA_\kappa -\frac{4M_z^2}{\bar{g}^2s}\lambda s \frac{t_\beta}{1+t_\beta^2}\right] \hspace{1cm} \\
  \ea


where we have also used,

\ba \fp{\mu_{eff}^2}{s} & = & 2 \lambda^2 s \hspace{1cm}
\fp{m_3^2}{s} =  \lambda (A_\lambda + 2\kappa s) \hspace{1cm}
\fp{c_\beta^2}{t_\beta} =  - \frac{2 t_\beta}{(t^2_\beta + 1)^2} \\
\fp{s_\beta^2}{t_\beta} & = & \frac{2 t_\beta}{(t^2_\beta + 1)^2} \hspace{1cm}
\fp{c_{2\beta}}{t_\beta}  = - \frac{4 t_\beta}{(t^2_\beta + 1)^2} \hspace{1cm}
\fp{s_{2\beta}}{t_\beta} = \frac{2- 2t^2_\beta}{(t^2_\beta + 1)^2} \ea


The coefficients from differentiating the reformulated EWSB conditions that are used to isolate $\mu_{eff}$ and $m_3^2$ are also rather simple,

\begin{equation} b_1 = - \frac{\lambda}{s} \hspace{1cm}    b_2 = \frac{1}{2\lambda s^2}\frac{2t_\beta}{(t_\beta^2-1)^2} (m_{H_u}^2-m_{H_d}^2) \hspace{1cm}  b_3 =  -\frac{1}{4\lambda s^2} \end{equation}
and
\ba e_0 &=& \left[\frac{A_\lambda+\kappa s}{\lambda s}-2\sin{2\beta}\left(1+\frac{M_z^2}{\bar{g}^2s^2}\right) \right] \hspace{1cm} 
e_1  = -\frac{2\lambda s\sin{2\beta}-(A_\lambda+2\kappa s)}{s^2} \hspace{1cm}\\
e_2  &=& - \frac{1-t_\beta^2}{t_\beta(1+t_\beta^2)}\frac{A_\lambda+\kappa s}{s} \hspace{3.7cm} 
e_3 =  -\frac{\lambda\sin{2\beta}}{\bar{g}^2s^2} \hspace{1cm} 
e_4 = 1 \hspace{1cm}\ea
\begin{eqnarray}
	0&=&\left[-(A_\lambda+\kappa s)s+2\lambda\sin{2\beta}(s^2+M_z^2/\bar{g}^2)\right]d\lambda +\left[2\lambda^2 s\sin{2\beta} -\lambda(A_\lambda+2\kappa s)\right]ds\notag\\
	&&+ \frac{1-t^2}{t(1+t^2)}\lambda s(A_\lambda+\kappa s)dt+ \frac{\lambda^2}{\bar{g}^2} \sin{2\beta}dM_z^2 -\lambda s^2d\kappa \\
	&=&\left[\frac{A_\lambda+\kappa s}{\lambda s}-2\sin{2\beta}\left(1+\frac{M_z^2}{\bar{g}^2s^2}\right) \right]d\lambda -\frac{2\lambda s\sin{2\beta}-(A_\lambda+2\kappa s)}{s^2}ds\notag\\
	&&- \frac{1-t^2}{t(1+t^2)}\frac{A_\lambda+\kappa s}{s}dt -\frac{\lambda\sin{2\beta}}{\bar{g}^2s^2} dM_z^2 +d\kappa\\
	&\equiv& e_0d\lambda+ e_1ds + e_2dt + e_3dM_z^2 +e_4d\kappa, \label{dkappa}
\end{eqnarray}


\begin{eqnarray}
	dm_S^2 &=& -\frac{4M_z^2}{\bar{g}^2s}\left[\lambda s-\frac{t}{1+t^2}(A_\lambda+\kappa s)\right]d\lambda-\left(4\kappa^2s+\kappa A_\kappa+\frac{4M_z^2}{\bar{g}^2s^2}\frac{t}{1+t^2}\lambda A_\lambda\right)ds\notag\\
	&&+\frac{4M_z^2}{\bar{g}^2s^2}\frac{1-t^2}{(1+t^2)^2}~\lambda s(A_\lambda+\kappa s)dt -\left[2\lambda^2/\bar{g}^2-\frac{4\lambda}{\bar{g}^2s}\frac{t}{1+t^2}(A_\lambda+\kappa s)\right]dM_z^2\notag\\
	&&-\left[4\kappa s^2+sA_\kappa -\frac{4M_z^2}{\bar{g}^2s}\lambda s \frac{t}{1+t^2}\right]d\kappa\\
	&\equiv&a^s_0d\lambda + a^s_1ds + a^s_2dt + a^s_3dM_z^2 + a^s_4d\kappa.\label{dms1}
\end{eqnarray}
% subsection jacobian_of_t__lambdakappa_m_S_ (end)
Finally it also useful to re-express $dm_S^2$ in two different ways.  First we substitute in for $d \lambda$ and $d\kappa$ in Eq.~(\ref{Ap:dms1}) so that it can be rewritten as:
\begin{eqnarray}
	dm_S^2	&\equiv& f_1ds + f_2dt_\beta+ f_3dM_z^2.\label{Ap:dms2} \\
        f_1	&=&\frac{1}{e_4}\left(b_1(a^s_0e_4-a^s_4 e_0)+(a^s_1e_4-a^s_4 e_1)\right)\notag \\
f_2 &=&  \frac{1}{e_4}\left(b_2(a^s_0e_4-a^s_4 e_0)+(a^s_2e_4-a^s_4 e_2)\right) \notag\\
f_3	&=&\frac{1}{e_4}\left(b_3(a^s_0e_4-a^s_4 e_0)+(a^s_3e_4-a^s_4 e_3)\right) \notag
\end{eqnarray}  and then we make an alternative substitution for $ds$ and $dt_\beta$ giving,
\begin{eqnarray}
	dm_S^2
	&\equiv&h_0d\lambda+h_3 dM_z^2+h_4 d\kappa. \\
 h_0 &=&-\left[-\frac{f_1}{b_1}+\left(f_2-\frac{b_2}{b_1}f_1\right)\frac{-e_1-b_1e_0}{b_2e_1-b_1e_2}\right]\notag\\
  h_3 &=&+\left[\left(f_3-\frac{b_3}{b_1}f_1\right)-\left(f_2-\frac{b_2}{b_1}f_1\right)\frac{b_3e_1-b_1e_3}{b_2e_1-b_1e_2}\right]\notag\\
 h_4 &=&+\left(f_2-\frac{b_2}{b_1}f_1\right)\frac{b_1e_4}{b_2e_1-b_1e_2}d\kappa\notag
\end{eqnarray}


The Jacobian matrix is the written as 

\begin{eqnarray}
	J_{\mathcal{T}_{\kappa m_S}}
	&=&
	\begin{vmatrix}
		& a_s^{H_u} & a_{M_Z^2}^{H_u}  & a_{\tan \beta}^{H_u}   &\\
		& a_s^{H_d} &  a_{M_Z^2}^{H_d} & a_{\tan \beta}^{H_d}  &\\
		& a_s^s  &  a_{M_Z^2}^s  & a_{\tan \beta}^s  &
	\end{vmatrix},
\end{eqnarray} where the coefficients are

 



\end{appendix}

\end{color}
